DreamScene: 3D Gaussian-based Text-to-3D Scene Generation via Formation Pattern Sampling

Text-to-3D scene generation holds immense potential for the gaming, film, and architecture sectors. Despite significant progress, existing methods struggle with maintaining high quality, consistency, and editing flexibility. In this paper, we propose DreamScene, a 3D Gaussian-based novel text-to-3D scene generation framework, to tackle the aforementioned three challenges mainly via two strategies. First, DreamScene employs Formation Pattern Sampling (FPS), a multi-timestep sampling strategy guided by the formation patterns of 3D objects, to form fast, semantically rich, and high-quality representations. FPS uses 3D Gaussian filtering for optimization stability, and leverages reconstruction techniques to generate plausible textures. Second, DreamScene employs a progressive three-stage camera sampling strategy, specifically designed for both indoor and outdoor settings, to effectively ensure object-environment integration and scene-wide 3D consistency. Last, DreamScene enhances scene editing flexibility by integrating objects and environments, enabling targeted adjustments. Extensive experiments validate DreamScene's superiority over current state-of-the-art techniques, heralding its wide-ranging potential for diverse applications. Code and demos will be released at https://dreamscene-project.github.io .

==> main_bbl.tex <==
\begin{thebibliography}{10}
\providecommand{\url}[1]{\texttt{#1}}
\providecommand{\urlprefix}{URL }
\providecommand{\doi}[1]{https://doi.org/#1}

\bibitem{barron2021mip}
Barron, J.T., Mildenhall, B., Tancik, M., Hedman, P., Martin-Brualla, R., Srinivasan, P.P.: Mip-nerf: A multiscale representation for anti-aliasing neural radiance fields. In: Proceedings of the IEEE/CVF International Conference on Computer Vision. pp. 5855--5864 (2021)

\bibitem{chen2024survey}
Chen, G., Wang, W.: A survey on 3d gaussian splatting. arXiv preprint arXiv:2401.03890  (2024)

\bibitem{chen2023fantasia3d}
Chen, R., Chen, Y., Jiao, N., Jia, K.: Fantasia3d: Disentangling geometry and appearance for high-quality text-to-3d content creation. arXiv preprint arXiv:2303.13873  (2023)

\bibitem{cohen2023set}
Cohen-Bar, D., Richardson, E., Metzer, G., Giryes, R., Cohen-Or, D.: Set-the-scene: Global-local training for generating controllable nerf scenes. arXiv preprint arXiv:2303.13450  (2023)

\bibitem{fan2023lightgaussian}
Fan, Z., Wang, K., Wen, K., Zhu, Z., Xu, D., Wang, Z.: Lightgaussian: Unbounded 3d gaussian compression with 15x reduction and 200+ fps. arXiv preprint arXiv:2311.17245  (2023)

\bibitem{guo2023threestudio}
Guo, Y.C., Liu, Y.T., Wang, C., Zou, Z.X., Luo, G., Chen, C.H., Cao, Y.P., Zhang, S.H.: threestudio: A unified framework for 3d content generation (2023)

\bibitem{hertz2022prompt}
Hertz, A., Mokady, R., Tenenbaum, J., Aberman, K., Pritch, Y., Cohen-Or, D.: Prompt-to-prompt image editing with cross attention control. arXiv preprint arXiv:2208.01626  (2022)

\bibitem{ho2020denoising}
Ho, J., Jain, A., Abbeel, P.: Denoising diffusion probabilistic models. Advances in neural information processing systems  \textbf{33},  6840--6851 (2020)

\bibitem{ho2022classifier}
Ho, J., Salimans, T.: Classifier-free diffusion guidance. arXiv preprint arXiv:2207.12598  (2022)

\bibitem{hollein2023text2room}
H{\"o}llein, L., Cao, A., Owens, A., Johnson, J., Nie{\ss}ner, M.: Text2room: Extracting textured 3d meshes from 2d text-to-image models. arXiv preprint arXiv:2303.11989  (2023)

\bibitem{huang2023dreamtime}
Huang, Y., Wang, J., Shi, Y., Qi, X., Zha, Z.J., Zhang, L.: Dreamtime: An improved optimization strategy for text-to-3d content creation. arXiv preprint arXiv:2306.12422  (2023)

\bibitem{hwang2023text2scene}
Hwang, I., Kim, H., Kim, Y.M.: Text2scene: Text-driven indoor scene stylization with part-aware details. In: Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition. pp. 1890--1899 (2023)

\bibitem{jun2023shap}
Jun, H., Nichol, A.: Shap-e: Generating conditional 3d implicit functions. arXiv preprint arXiv:2305.02463  (2023)

\bibitem{kerbl20233d}
Kerbl, B., Kopanas, G., Leimk{\"u}hler, T., Drettakis, G.: 3d gaussian splatting for real-time radiance field rendering. ACM Transactions on Graphics  \textbf{42}(4) (2023)

\bibitem{lee2023compact}
Lee, J.C., Rho, D., Sun, X., Ko, J.H., Park, E.: Compact 3d gaussian representation for radiance field. arXiv preprint arXiv:2311.13681  (2023)

\bibitem{li2023sweetdreamer}
Li, W., Chen, R., Chen, X., Tan, P.: Sweetdreamer: Aligning geometric priors in 2d diffusion for consistent text-to-3d. arXiv preprint arXiv:2310.02596  (2023)

\bibitem{liang2023luciddreamer}
Liang, Y., Yang, X., Lin, J., Li, H., Xu, X., Chen, Y.: Luciddreamer: Towards high-fidelity text-to-3d generation via interval score matching. arXiv preprint arXiv:2311.11284  (2023)

\bibitem{lin2023magic3d}
Lin, C.H., Gao, J., Tang, L., Takikawa, T., Zeng, X., Huang, X., Kreis, K., Fidler, S., Liu, M.Y., Lin, T.Y.: Magic3d: High-resolution text-to-3d content creation. In: Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition. pp. 300--309 (2023)

\bibitem{lin2023componerf}
Lin, Y., Bai, H., Li, S., Lu, H., Lin, X., Xiong, H., Wang, L.: Componerf: Text-guided multi-object compositional nerf with editable 3d scene layout. arXiv preprint arXiv:2303.13843  (2023)

\bibitem{liu2023zero}
Liu, R., Wu, R., Van~Hoorick, B., Tokmakov, P., Zakharov, S., Vondrick, C.: Zero-1-to-3: Zero-shot one image to 3d object. In: Proceedings of the IEEE/CVF International Conference on Computer Vision. pp. 9298--9309 (2023)

\bibitem{metzer2023latent}
Metzer, G., Richardson, E., Patashnik, O., Giryes, R., Cohen-Or, D.: Latent-nerf for shape-guided generation of 3d shapes and textures. In: Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition. pp. 12663--12673 (2023)

\bibitem{mildenhall2021nerf}
Mildenhall, B., Srinivasan, P.P., Tancik, M., Barron, J.T., Ramamoorthi, R., Ng, R.: Nerf: Representing scenes as neural radiance fields for view synthesis. Communications of the ACM  \textbf{65}(1),  99--106 (2021)

\bibitem{mokady2023null}
Mokady, R., Hertz, A., Aberman, K., Pritch, Y., Cohen-Or, D.: Null-text inversion for editing real images using guided diffusion models. In: Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition. pp. 6038--6047 (2023)

\bibitem{muller2022instant}
M{\"u}ller, T., Evans, A., Schied, C., Keller, A.: Instant neural graphics primitives with a multiresolution hash encoding. ACM Transactions on Graphics (ToG)  \textbf{41}(4),  1--15 (2022)

\bibitem{nichol2022point}
Nichol, A., Jun, H., Dhariwal, P., Mishkin, P., Chen, M.: Point-e: A system for generating 3d point clouds from complex prompts. arXiv preprint arXiv:2212.08751  (2022)

\bibitem{ouyang2023text2immersion}
Ouyang, H., Heal, K., Lombardi, S., Sun, T.: Text2immersion: Generative immersive scene with 3d gaussians. arXiv preprint arXiv:2312.09242  (2023)

\bibitem{park2019deepsdf}
Park, J.J., Florence, P., Straub, J., Newcombe, R., Lovegrove, S.: Deepsdf: Learning continuous signed distance functions for shape representation. In: Proceedings of the IEEE/CVF conference on computer vision and pattern recognition. pp. 165--174 (2019)

\bibitem{po2023compositional}
Po, R., Wetzstein, G.: Compositional 3d scene generation using locally conditioned diffusion. arXiv preprint arXiv:2303.12218  (2023)

\bibitem{poole2022dreamfusion}
Poole, B., Jain, A., Barron, J.T., Mildenhall, B.: Dreamfusion: Text-to-3d using 2d diffusion. arXiv preprint arXiv:2209.14988  (2022)

\bibitem{ramesh2022hierarchical}
Ramesh, A., Dhariwal, P., Nichol, A., Chu, C., Chen, M.: Hierarchical text-conditional image generation with clip latents. arXiv preprint arXiv:2204.06125  \textbf{1}(2), ~3 (2022)

\bibitem{rombach2022high}
Rombach, R., Blattmann, A., Lorenz, D., Esser, P., Ommer, B.: High-resolution image synthesis with latent diffusion models. In: Proceedings of the IEEE/CVF conference on computer vision and pattern recognition. pp. 10684--10695 (2022)

\bibitem{saharia2022photorealistic}
Saharia, C., Chan, W., Saxena, S., Li, L., Whang, J., Denton, E.L., Ghasemipour, K., Gontijo~Lopes, R., Karagol~Ayan, B., Salimans, T., et~al.: Photorealistic text-to-image diffusion models with deep language understanding. Advances in Neural Information Processing Systems  \textbf{35},  36479--36494 (2022)

\bibitem{shen2021deep}
Shen, T., Gao, J., Yin, K., Liu, M.Y., Fidler, S.: Deep marching tetrahedra: a hybrid representation for high-resolution 3d shape synthesis. Advances in Neural Information Processing Systems  \textbf{34},  6087--6101 (2021)

\bibitem{shi2023mvdream}
Shi, Y., Wang, P., Ye, J., Long, M., Li, K., Yang, X.: Mvdream: Multi-view diffusion for 3d generation. arXiv preprint arXiv:2308.16512  (2023)

\bibitem{song2020denoising}
Song, J., Meng, C., Ermon, S.: Denoising diffusion implicit models. arXiv preprint arXiv:2010.02502  (2020)

\bibitem{tang2023dreamgaussian}
Tang, J., Ren, J., Zhou, H., Liu, Z., Zeng, G.: Dreamgaussian: Generative gaussian splatting for efficient 3d content creation. arXiv preprint arXiv:2309.16653  (2023)

\bibitem{vilesov2023cg3d}
Vilesov, A., Chari, P., Kadambi, A.: Cg3d: Compositional generation for text-to-3d via gaussian splatting. arXiv preprint arXiv:2311.17907  (2023)

\bibitem{wang2024prolificdreamer}
Wang, Z., Lu, C., Wang, Y., Bao, F., Li, C., Su, H., Zhu, J.: Prolificdreamer: High-fidelity and diverse text-to-3d generation with variational score distillation. Advances in Neural Information Processing Systems  \textbf{36} (2024)

\bibitem{yi2023gaussiandreamer}
Yi, T., Fang, J., Wu, G., Xie, L., Zhang, X., Liu, W., Tian, Q., Wang, X.: Gaussiandreamer: Fast generation from text to 3d gaussian splatting with point cloud priors. arXiv preprint arXiv:2310.08529  (2023)

\bibitem{yu2023text}
Yu, X., Guo, Y.C., Li, Y., Liang, D., Zhang, S.H., Qi, X.: Text-to-3d with classifier score distillation. arXiv preprint arXiv:2310.19415  (2023)

\bibitem{zhang2024text2nerf}
Zhang, J., Li, X., Wan, Z., Wang, C., Liao, J.: Text2nerf: Text-driven 3d scene generation with neural radiance fields. IEEE Transactions on Visualization and Computer Graphics  (2024)

\bibitem{zhang2023scenewiz3d}
Zhang, Q., Wang, C., Siarohin, A., Zhuang, P., Xu, Y., Yang, C., Lin, D., Zhou, B., Tulyakov, S., Lee, H.Y.: Scenewiz3d: Towards text-guided 3d scene composition. arXiv preprint arXiv:2312.08885  (2023)

\bibitem{zhao2023survey}
Zhao, W.X., Zhou, K., Li, J., Tang, T., Wang, X., Hou, Y., Min, Y., Zhang, B., Zhang, J., Dong, Z., et~al.: A survey of large language models. arXiv preprint arXiv:2303.18223  (2023)

\bibitem{zhou2024gala3d}
Zhou, X., Ran, X., Xiong, Y., He, J., Lin, Z., Wang, Y., Sun, D., Yang, M.H.: Gala3d: Towards text-to-3d complex scene generation via layout-guided generative gaussian splatting. arXiv preprint arXiv:2402.07207  (2024)

\end{thebibliography}

==> sec/10_limitation.tex <==
\section{Limitation}
%Dreamscene目前在室外场景中无法像Text2Room和Text2Scene生成非常接近真实的环境。这是由于他们的方法是通过图片inpainting的方法进行生成，所以其观察相机位姿非常有限，整个场景的3D一致性很差。而我们为了保证整个场景一致，牺牲了一部分真实性。后续工作我们会引入深度监督，引导室外场景可以像室内一样生成风格更加真实。
\sysname currently cannot generate outdoor scenes as realistically close to actual environments as Text2Room~\cite{hollein2023text2room} and Text2NeRF~\cite{zhang2024text2nerf}. This is because their methods generate scenes through image inpainting, resulting in very limited observable camera poses and poor 3D consistency across the entire scene. In contrast, we sacrificed a degree of realism to ensure overall scene consistency. In future work, we plan to incorporate depth supervision to guide the generation of outdoor scenes with a style as realistic as indoor ones.

==> sec/5_conclusion.tex <==

\section{Conclusion}
%在这篇文章中，我们提出了一个新颖的基于3D高斯的文本到3D场景的生成策略，通过一个的高效文生3D的策略,相机路径采样策略和物体环境的组合场景方式，解决目前3D场景生成方法低效，不一致和只能有限编辑问题。大量的实验证明了DreamScene是3D场景生成中里程碑的工作，将会在很多领域有着广阔的应用。
In this paper, we introduce a novel Text-to-3D Ccene generation strategy \sysname. By employing an efficient Text-to-3D generation strategy, a Camera Sampling Trajectory, combining objects and environments, we address the current issues of inefficiency, inconsistency, and limited editability in current Text-to-3D Scene generation methods. Extensive experiments have demonstrated that \sysname\ is a milestone achievement in 3D scene generation, poised for wide-ranging applications across numerous fields.








==> sec/7_implementation_details.tex <==
\section{Implementation Details}
%我们使用GPT4作为我们场景提示分解的语言大模型,point-E生成的稀疏点云作为物体的初始化,Stable Diffusion v2-1 base作为我们的2D引导文生图模型,单目图像深度估计模型g_D为ZoeDepth。物体的最大迭代次数max iter为3000轮，环境最大迭代次数为5000轮，时间间隔初始值m为5，每800轮下降1，压缩比例gamma为60%。k_in = k_out = 4我们在英伟达RTX3090服务器上进行实验，单个物体生成需要一个小时，场景生成需要一个小时。（Lucid Dreamer中DDIM后退说不说？）
We utilize GPT-4 as our language large model for scene prompt decomposition, Point-E generated sparse point clouds for the initial representation of objects,  Stable Diffusion v2-1 base as our 2D guidance text-to-image model, and ZoeDepth as  the monocular image depth estimation model $g_D$. The maximum number of iterations for objects $max iter$ is set to 3000 rounds, and the environment is set to 5000 rounds. The initial time interval value, $m$, starts at 5 and decreases by 1 every 800 rounds, with a compression ratio gamma of 60\%. Both $k_{in}$ and $k_{out}$ are set to 4. We conduct our experiments on an NVIDIA GeForce RTX 3090 GPU, with individual object generation taking one hour and scene generation taking also one hour.


==> sec/9_supplement_material.tex <==

\section{Discussions of Current Methods}

% Current text-to-3D scene generation methods, as illustrated in Fig.~\ref{fig:compare} face significant limitations. Methods~\cite{zhang2024text2nerf,hollein2023text2room,ouyang2023text2immersion} relying on inpainted images for scene completion can generate realistic visuals but suffer from limited 3D consistency of the generated scenes. Even minor disturbances can lead to the collapse of the scene's visual integrity, indicating a lack of robustness. Moreover, such methods typically do not allow for the editing of objects within the scene and have unrealistic scene compositions, such as a living room cluttered with an excessive number of sofas. 
% While some methods~\cite{cohen2023set,zhang2023scenewiz3d}, akin to ours, attempt to merge objects with environments for achieving a degree of consistency, they generally yield scenes of lower quality and can accommodate only a limited number of objects. Approaches \cite{vilesov2023cg3d,zhou2024gala3d,lin2023componerf} focusing solely on object combination fall short of generating comprehensive scenes. The constraints on quality, consistency, and editability have thus far hindered the broader application of text-to-3D technologies. Our method represents a leap forward by ensuring high-quality, scene-wide consistency and enabling flexible editing.

% Text2NeRF
% 1.场景初始化。通过2d文本到图像的扩散模型生成初始视图I，同时估计深度图D。通过视图I和深度图D构建三维NeRF表示。采用基于深度图像的渲染（DIBR）方法构建支持集S0来避免缺乏多视角监督的过拟合和几何模糊问题。
% 2.文本驱动的inpainting。除了初始视图I0之外的渲染结果具有缺失的内容。为了补充缺失的区域，采用了一种基于预训练扩散模型fd的文本驱动修复方法。对每个要完成的视图I R k执行多次修复过程，并从所有候选inpainting结果中选择与CLIP语义空间中的初始视图最相似的一个。
% 3.深度对齐。与初始视图的深度图D0不同，DEk不能直接作为更新辐射场的监督，因为它是独立预测的，并且可能与重叠区域中的已知深度图冲突。所以需要进行深度对齐的操作。
% 4.渐进式修复和更新。将先前修复的内容反映到下一个视图中，实现修复结果。


% Text2NeRF, Text2Room, Text2Immersion
%这类方法通常是通过图像补全的生成的场景，他们首先会初始化一张图像，然后遮挡一部分，作为旋转到另外角度的视角，利用补全的模型（如xxx）和深度监督，生成出遮挡部分的图片和对应的估计深度，通过对齐深度和图像往复生成整个场景，并在最后填补场景中的空缺。(再详细一点)

% 此类方法虽然在训练时的相机位置上（例如场景中心）能够获得良好的视觉效果，但其可见范围具有很大的局限性。一旦超出训练中的相机区域就会导致场景崩溃（如论文中图4a所示）这代表他们不具有scene-wide的3D一致性。同时，这种方法还会导致环境中的某些物体重复出现多次。比如客厅中的沙发等等等等。这代表他们的合理性也较差。相关视频结果我们放在了补充材料的压缩包中，每种方法的视频以各自的名字命名。


%These methods, as delineated in references such as Zhang et al. 2024, Hollein et al. 2023, and Ouyang et al. 2023, predominantly employ text-to-image inpainting for scene generation. The process begins with the initialization of an image, which is then partially masked to represent a view from an alternate angle. Leveraging pretrained image inpainting models like Stable Diffusion, alongside depth supervision, they reconstruct the occluded image segments and deduce their depths, thus iteratively composing the entire scene through depth and image alignment. While these techniques are adept at producing visually appealing outcomes at specific training camera positions, such as the scene's center, they encounter significant limitations in visible range. Venturing beyond the predefined camera areas used during training precipitates scene degradation, as exemplified in Fig. 4a, underscoring a deficiency in scene-wide 3D consistency. Concurrently, this method's tendency to replicate certain environmental objects, like the proliferation of sofas in a living room scenario, highlights issues with logical scene composition. Supplementary material, including videos demonstrating each method, is compiled in a dedicated compressed package, with files named accordingly.

\noindent\textbf{Inpainting-based methods} employ text-to-image inpainting for scene generation~\cite{zhang2024text2nerf,hollein2023text2room,ouyang2023text2immersion}. They first initialize an image and then partially mask it to represent a view from an alternate angle. Leveraging pretrained image inpainting models like Stable Diffusion~\cite{rombach2022high}, alongside depth estimation, they reconstruct the occluded image segments and deduce their depths, iteratively composing the entire scene through depth and image alignment. While such methods can achieve good visual effects at the camera positions (e.g., the center of the scene) during the generation process, they encounter significant limitations in visible range. Venturing beyond the predefined camera areas used during generation precipitates scene degradation, as exemplified in Fig.~\textcolor{red}{4a} of the paper, underscoring a deficiency in scene-wide 3D consistency. Concurrently, this method's tendency to replicate certain environmental objects, like the proliferation of sofas in a living room scenario, highlights issues with logical scene composition. 
%Supplementary material, including videos demonstrating each method, is compiled in a dedicated compressed package, with files named accordingly.


% text2room 的深度补全:Gwangbin Bae, Ignas Budvytis, and Roberto Cipolla. Irondepth: Iterative refinement of single-view depth using surface normal and its uncertainty. In British Machine Vision Conference (BMVC), 2022. 3, 5

%\subsubsection{\textcolor{red}{Combination-based} methods.}

% 这些方法同样使用组合方式来构建场景，但是由于其基础的生成方法生成质量低下，训练速度缓慢，所以导致了较差的场景生成结果。同时有的方法使用不同的三维表示（例如nerf+DMTet）来组合物体和场景，这增加了场景表示的复杂程度，所以在场景中放置的物体数量十分有限（2-3个），对其应用带来了不利影响。而DreamScene中的 Formation Patttern Sampling(FPS)可以在极短时间内生成高质量的3D内容，可以只使用一种3D表示组合成整个场景，场景中可以放置20个以上的物体。

\noindent\textbf{Combination-based methods} also employ a combination approach to construct scenes~\cite{cohen2023set,zhang2023scenewiz3d}. However, they face challenges including low generation quality and slow training speeds. Moreover, \cite{zhang2023scenewiz3d} utilizes various 3D representations (such as NeRF$+$DMTet) to \textcolor{red}{integrate objects and scenes}, increasing the complexity of scene representation and thus limiting the number of objects that can be placed within the scene (2-3 objects), impacting their applicability. In contrast, \sysname's Formation Pattern Sampling (FPS) can generate high-quality 3D content in a very short time, using a single 3D representation to compose the entire scene, allowing for more than 20 objects to be placed within the scene. This underscores \sysname's remarkable superiority.


%Some past methods~\cite{cohen2023set,zhang2023scenewiz3d} also use combining objects and environments to build scenes, some of them use 3D representations that are difficult to merge, training slowly and with poor generation quality, and some even use different 3D representations between objects and environments, which greatly increases the complexity of the system and adversely affects the application of 3D assets. At the same time, their initialization methods often only consider indoor scenes, which also leads to poor generation results.
% 使用，
% Set-the-Scene SceneWiz3D
%表示方法不好，SceneWiz3D甚至使用不同的三维表示进行组合，非常复杂。效果质量差。

%初始化方式不行，只考虑了室内，室外效果很差。

%\subsubsection{\textcolor{red}{Objects combination methods}.}
% Methods~\cite{vilesov2023cg3d,zhou2024gala3d,lin2023componerf}
% GALA3D?
% 此类方法没有考虑环境场景，只考虑物体组合是否合理，他们所生成的并不能算是一个完整的场景，而是一些物体的简单组合。我们认为场景的组合方式应该更加多样化并且具有更好的可控性。
\noindent\textbf{Objects combination  methods} do not take the environmental context into account, focusing solely on whether the combination of objects is logical~\cite{zhou2024gala3d,vilesov2023cg3d,lin2023componerf}. They generate a simple assembly of objects rather than a complete scene. We believe that the approach to scene composition should be more diverse and offer greater controllability.

%\subsubsection{Other methods}
%Methods~\cite{wang2024prolificdreamer}

% DreamScene可以高效，一致，编辑灵活的生成3D场景，与以上方法相比体现了巨大的优势。
\par \sysname\ demonstrates a significant advantage by efficiently, consistently, and flexibly generating 3D scenes, showcasing a substantial superiority over the aforementioned methods. Please refer to the supplemental comparison videos of the methods mentioned in the paper at the \textit{comparison results} folder. Due to space limitations, we put our results at the \textit{scene results} folder.
%
\section{Additional Implementation Details}
% \subsection{Camera Sampling}
The overall generation process of \sysname\ is shown in Algorithm~\ref{alg:DreamScene}.

\subsection{Rendering and Training Settings}

We render images with a size of 512×512 for optimization. During the optimization process, we do not reset the opacity, to maintain the consistency of the optimization during the training process and avoid gradient disappearance due to opacity reset.

% 我们渲染尺寸为512×512的图像用于训练，在优化过程中，我们不会重置不透明度，这能够让我们在训练过程中保持优化的一致性，避免出现由于不透明度重置导致的梯度消失。


% 在粗优化阶段，每次迭代我们采样4个相机用于优化，并且随机扰动背景颜色等，增加多样性。我们的什么什么区间从多少线性下降到多少，由于我们的方法的优势，我们的形状形成很迅速。

% 在重建阶段，我们将关闭所有扰动以免影响重建效果，在不同的高度上环绕物体采样相机，确保物体的外表面均能被覆盖，并获得最佳的伪GT图像，这一阶段我们的loss置为多少多少。



% 室外：





% 室内：
% 在第一阶段，我们冻结地面和物体参数，但会将物体渲染到场景中。与室外相似，我们主要围绕场景中心采样相机，但半径被设置为尽量大的值，尽量将所有物体包含在内，从而减少场景的多头问题，此时的相机俯仰角在75~115之间。在一定阶段后，我们会对物体周边采样相机，从而减少物体遮挡对环境造成的影响。（理论上讲这里也可以加上一些在格子区域中采样的）
% 在第二阶段，我们冻结环境参数，开始优化地面参数。室内的相机采样策略基本不变，但会改变俯仰角到45~90之间以获得对地面的覆盖。同时会增加物体周边的采样和从场景中心向周边的采样，从而改善地面与墙壁之间的融合。
% 在第三阶段，我们对环境和地面都进行优化，同样将前面两个阶段所用到的相机位姿综合起来使用，使场景中的区域得到均匀全面的覆盖，从而获得良好的重建效果。

\begin{algorithm}
\caption{\sysname}
\label{alg:DreamScene}
\begin{algorithmic}[1] % 数字1表示每一行都显示数字
%\Procedure{MyProcedure}{$a,b$} % 算法的标题
%\State Efficient Generation of Single Objects
\State $Y \rightarrow y_1,y_2,...,y_N,y_e$;
\For{$n = [1,2,...,N,e]$}
    \If{$n$ is not $e$}
        \State Initialize 3D Gaussian of $obj_n$ 
    \Else
        \State Initialize 3D Gaussian of environment
        % \State Initialize camera path 
    \EndIf
    % \State Set a threshold $max_\theta$ for points number of 3D Gaussian $num_\theta$
    \For{$iter = [0,1,...,max\_iter]$}
        \If{$n$ is not $e$}
            \State Sample camera pose $c$
        \Else
            \State Sample camera pose $c$ follow strategy in Sec.~\ref{camera_sampling}
        \EndIf
        \State $x_0 = g(\theta,c)$
        \State $T_{end} = (1-\frac{iter}{max\_iter}) timesteps$
        \For{$i = [1,2,...,m]$}
            \State $t_i = T_{end}\cdot random(\frac{i-1}{m},\frac{i}{m})$
            \State $x_i=DDIM_(x_{i-1},i)$
            \State $\epsilon_{\phi}(x_{i}; y_n, t_i) = $U-Net$(x_i,y,t_i)$
            \State $\epsilon_{\phi}(x_i; \emptyset, t_i) = $U-Net$(x_i,\emptyset,t_i)$ 
        \EndFor
        \State $\nabla_{\theta}\mathcal{L}_{\text{MTS}}(\theta) = \mathbb{E}_{t,\epsilon,c}\left[\sum\limits_{i=1}^{m} w(t)(\epsilon_{\phi}(x_{t_i}; y_n, t_i) - \epsilon_{\phi}(x_{t_i}; \emptyset, t_i))\frac{\partial g(\theta,c)}{\partial \theta}\right]$
        \State Update $\theta$
        \If{$iter\%compress\_iter$}
        % \If{$num_\theta > max_\theta$}
        \State $Score_k = \sum_{j=1}^{H\times W \times M} \frac{V(k)}{D(r_j,k)^2\times maxV(r_j)} $
        \State $Sort(Score_k)$
        \State Delete last $z$ 3D Gaussians
        \EndIf
    \EndFor
    \If{$n$ is $e$}
        \State Save 3D Gaussian Representation of the Scene
        \State break
    \EndIf
    \State Save 3D Gaussian Representation $obj_n$ of text $y_n$
    \State $world(x) = r\cdot s \cdot obj_n(x) + t$
    \State Add $obj_n$ to the Scene
\EndFor
%\State  Scene Generation
%\EndProcedure
\end{algorithmic}
\end{algorithm}

\subsection{Camera Sampling Strategy}
\label{camera_sampling}
This section outlines a three-stage camera sampling strategy for crafting both outdoor and indoor scenes. The process is as follows:
% leveraging techniques for optimizing environments and ground parameters
\subsubsection{Outdoor}
\begin{itemize}
% 在第一阶段，我们在场景中心附近采样相机，冻结地面和物体参数，不渲染物体，仅优化周围环境。这个阶段我们将相机的俯仰角设定在80~110之间，到70%的轮数后我们在相机采样中，即在一次采样4个相机，4个相机指向同一方向，分别位于场景中心两侧，距离为半径的1/4或1/2，这能够让环境在不同距离上都获得较好的视觉效果。同时，我们在相机高度上加入了一定的随机性，相机的位置将在盒子的中心附近随机。
\item In the first stage, we freeze the parameters of the ground and objects, focusing solely on optimizing the surrounding environments without rendering the objects. During this phase, we sample cameras near the center of the scene, the camera's pitch angle is set between 80 to 110 degree. After reaching 70\% of the iterations of this stage, we select four camera poses for multi-camera sampling at each later iteration. These four cameras, all directed towards the same direction, are positioned on either side of the scene center at distances of either 1/4 or 1/2 of the radius, ensuring the environments achieve satisfactory visual effects across various distances.


    % \item  Cameras are sampled near the scene center, with ground and object parameters frozen and objects not rendered, focusing only on optimizing the surrounding environment. The camera's pitch angle is set between 80-110 degrees. After 70\% of the rounds, multi-segment optimization is introduced by sampling four cameras pointing in the same direction, positioned on either side of the scene center at distances of 1/4 or 1/2 of the radius to enhance visual effects at varying distances. The camera height includes some randomness, with positions near the center of a box.

% 在第二阶段，我们冻结周围环境参数，同样不渲染物体，仅优化地面参数。我们同样每次采样一个训练迭代中的4个相机，与第一阶段的后期采样策略相似，俯仰角也调整到85~95之间，这样能够减少单一的地面或单一的环境出现在渲染图像中，从而改善场景生成的效果。
\item In the second stage, we freeze the parameters of the surrounding environments and objects, and focus solely on optimizing the ground without rendering objects. We sample four camera poses at each iteration, akin to the sampling strategy in the later part of the first stage. We adjust the pitch angle range to 85$\sim$95 degree, which can reduce the occurrence of a singular ground or environment in the rendered images, thereby enhancing the overall scene generation outcome.

% \item Surrounding environment parameters are frozen, and like Phase 1, only ground parameters are optimized without rendering objects. Four cameras are sampled per training iteration, similar to the late strategy of Phase 1, but without randomness in camera height and pitch angles adjusted to 85-95 degrees to minimize the appearance of monotonous ground or environment in rendered images, thus improving scene generation.

% 在第三阶段，我们对环境和地面都进行优化，并将物体渲染进场景中，从而获得协调统一的效果。我们把前面两个阶段所用到的相机位姿综合起来，这能够使场景中的区域得到均匀全面的覆盖，从而获得一致的重建结果。
\item In the third stage, we optimize both the surrounding environments and the ground, and render objects into the scene to achieve a harmonious and unified effect. We \textcolor{red}{integrate the camera positions used in the previous two stages}, ensuring that areas within the scene are evenly and comprehensively covered, thereby attaining a consistent reconstruction result.
    % \item Both environment and ground are optimized, and objects are rendered into the scene for a cohesive appearance. Camera poses from the previous phases are combined to ensure uniform coverage across the scene for optimal reconstruction.
\end{itemize}

\subsubsection{Indoor}
\begin{itemize}


% 在第一阶段，我们冻结地面和物体参数，并将物体渲染到场景中。我们主要围绕场景中心采样相机，半径被设置为尽量大的值，尽量将所有物体包含在内，从而减少场景的多头问题，此时的相机俯仰角在75~115之间。在一定阶段后，我们会对物体周边采样相机，从而减少物体遮挡对环境造成的影响。（理论上讲这里也可以加上一些在格子区域中采样的）
\item In the first stage, we freeze the ground and object parameters and \textbf{render} the objects into the scene. We primarily sample camera poses around the center of the scene and set the radius as large as possible to encompass all objects and thereby minimize the multi-head problem. At this stage, the pitch angle range of cameras is set to 75$\sim$115 degree. After the same iterations at outdoor settings, we sample camera poses around the objects to reduce the impact of object occlusion on the environment.

   % \item Similar to outdoors, ground and object parameters are frozen, but objects are rendered into the scene. Cameras are primarily sampled around the center with a large radius to include all objects, reducing the multi-head problem with camera pitch angles between 75-115 degrees. Later, cameras are sampled around objects to minimize occlusion effects on the environment.

\item In the second stage, we freeze the environment parameters and begin optimizing the ground parameters. The indoor camera sampling strategy remains largely unchanged, but we adjust the pitch angle range to 45$\sim$90 degree to ensure coverage of the ground. Additionally, we increase the camera sampling around objects and from the center to the periphery of the scene, thereby enhancing the \textcolor{red}{integration between the ground and the walls}.

% 在第二阶段，我们冻结环境参数，开始优化地面参数。室内的相机采样策略基本不变，但会改变俯仰角到45~90之间以获得对地面的覆盖。同时会增加物体周边的采样和从场景中心向周边的采样，从而改善地面与墙壁之间的融合。


    % \item Environment parameters are frozen, focusing on optimizing ground parameters. The indoor camera sampling strategy remains similar, but pitch angles are adjusted to 45-90 degrees for ground coverage. Additional sampling around objects and from the center outwards improves the integration between ground and walls.

% 在第三阶段，我们对环境和地面都进行优化，同样将前面两个阶段所用到的相机位姿综合起来使用，使场景中的区域得到均匀全面的覆盖，从而获得良好的重建效果。
%\item In the third stage, we optimize both the environments and the ground, \textcolor{red}{integrating the camera positions used in the previous two stages}. This ensures that areas within the scene are evenly and comprehensively covered, leading to a satisfactory reconstruction outcome.

\item In the third stage, we optimize both the surrounding environments and the ground, and render objects into the scene in the same way as outdoor's.
%to achieve a harmonious and unified effects. We integrate the camera positions used in the previous two stages, ensuring that areas within the scene are evenly and comprehensively covered, thereby attaining a consistent reconstruction result.

    % \item Optimizes both environment and ground, integrating camera poses from earlier phases for even scene coverage and effective reconstruction.
\end{itemize}
% 在场景

Our indoor and outdoor camera sampling strategies correspond to typical bounded and unbounded scenes, respectively. For bounded scenes, we focus on ensuring consistency across various orientations. Hence we pay more attention to integrating objects with environments to avoid illogical layouts caused by generating excessive objects in the environment. For unbounded scenes, our primary concern lies with maintaining scene-wide consistency across varied distances. Therefore, we employ two different strategies for scene generation.

\section{Additional Results}

\subsection{Qualitative Results}
More qualitative results of FPS are shown in Fig.~\ref{fig:supp_object_result}.
More qualitative results of scene generation are shown in Fig.~\ref{fig:supp_outdoor_result} and Fig.~\ref{fig:supp_indoor_result}.
%补充材料视频中有更直观的结果展示。
%Please also refer to the supplemental videos at the \textit{object results} and the \textit{scene results} folder for a more visual demonstration.

%包含多个方向的图片. These results % 这些结果充分（）（）了我们的方法能够生成具有良好一致性和合理纹理的场景，并且能够满足用户对场景的风格要求。
% 这些结果体现了我们的方法在单物体和场景上均能够完成有效的生成并且取得当前最好的效果。

% \subsection{Objects}

\begin{figure}
\centering
\includegraphics[width=1\textwidth]{figures/object_rescale.pdf}

%上半部分是用训练时的相机渲染的结果，下图是场景内但不在训练集中的相机下渲染的结果
\caption{More object generation results of \sysname.
%Scene Results. The upper part shows images rendered using camera poses employed during the generation process, whereas the lower part shows the images rendered with the randomly selected camera poses within the scene.
}
\label{fig:supp_object_result}
\end{figure}

% \subsection{Scenes}

\begin{figure}
\centering
\includegraphics[width=1\textwidth]{figures/supp_scene_zoo.pdf}
\includegraphics[width=1\textwidth]{figures/supp_scene_park_.pdf}
\includegraphics[width=1\textwidth]{figures/supp_scene_space.pdf}
\includegraphics[width=1\textwidth]{figures/supp_scene_minecraft.pdf}
\caption{More outdoor scene generation results of \sysname.}
\label{fig:supp_outdoor_result}
\end{figure}

\begin{figure}
\centering
\includegraphics[width=1\textwidth]{figures/supp_scene_kitchen_eu.pdf}
\includegraphics[width=1\textwidth]{figures/supp_scene_bedroom_ukiyo_.pdf}
\includegraphics[width=1\textwidth]{figures/supp_scene_living_room.pdf}
\caption{More indoor scene generation results of \sysname.}
\label{fig:supp_indoor_result}
\end{figure}


\begin{figure}
\centering
\begin{subfigure}{0.3\linewidth}
\centering
\includegraphics[width=1\textwidth]{figures/Ablation1.pdf}
\caption{Randomly camera sampling}
\end{subfigure}
\hfill
\begin{subfigure}{0.3\linewidth}
\centering
\includegraphics[width=1\textwidth]{figures/Ablation2.pdf}
\caption{No distinction between environment and ground}
\end{subfigure}
\hfill
\begin{subfigure}{0.3\linewidth}
\centering
\includegraphics[width=1\textwidth]{figures/Ablation3.pdf}
\caption{\sysname\ three-stage camera sampling strategy}
\end{subfigure}
\vspace{-5pt}
\caption{The ablation results of different camera sampling strategies.}
\label{fig:sampling_ablation}
\end{figure}

\subsection{Ablation Study}
%如图所示，（a）是在场景中随机采样相机生成的场景图，由于很难保证场景中同一位置的多视角的一致性，所以优化过程往往会趋于崩溃（b）是使用由中心开始初始化到四周的策略，此时不区分环境和地面，可以看出来场景一致性有提高但是，地面与场景连接处生成效果不好，而且地面更容易出现粗大的高斯点（c）是使用了我们三阶段的策略，在保证了四周环境和地面的一致性的同时提高了生成质量。
% 补充消融？？？
Fig.~\ref{fig:sampling_ablation}(a) depicts a scene generated by randomly sampling cameras within the scene. Due to the difficulty in ensuring consistency of multi-angle views at the same location, the optimization process often tends to collapse. Fig.~\ref{fig:sampling_ablation}(b) utilizes a strategy that initiates from the center to the surroundings, where the environment and ground are not differentiated. It can be observed that while scene consistency improves, the connection between the ground and the scene is poorly generated, and the ground is prone to coarse Gaussian points. Fig.~\ref{fig:sampling_ablation}(c) employs our three-phase strategy, enhancing the generation quality while ensuring the consistency of the surrounding environment and ground.

==> sec/method2.tex <==
\subsection{HybridTime  Sampling}
Traditional score distillation sampling follows the training methodology of diffusion models \cite{ho2020denoising,song2020denoising,song2019generative}, employing random sampling of timesteps. DreamTime~\cite{huang2023dreamtime} posits that using a monotonically non-increasing function for timesteps sampling aligns the optimization of 3D models with the sampling process of diffusion models, thereby enhancing both the efficiency and quality of optimization. However, we have discovered that  hybridizing information from diffusion models across different timesteps  significantly enhances the convergence of the 3D representaion  and elevates the overall quality of its generation. We use pseudo-ground-truth(pseudoGT) images obtained from a single denoising step in lucidreamer~\cite{liang2023luciddreamer} to represent the information provided by the 2D Text-to-Image diffusion model at different timesteps t($0\sim 1000$).  We add $t$ timesteps of noise to the images $x_0$ to get $x_i$ and  estimate the  the pseudoGT images $\hat{x}_{0}^t$ using:
\begin{equation}
\hat{x}_{0}^t = \frac{x_{t} - \sqrt{1 - \bar{\alpha}_t} \epsilon_{\phi}(x_{t}, t, y)}{\sqrt{\bar{\alpha}_t}}.
\label{Eq:pseudoGT}
\end{equation}
As shown in Fig.\ref{fig:multi-timesteps},we discovered when timesteps $t$ is small, the 2D diffusion model provides the information of surface textures that are more detailed and realistic, and consistent with the current 3D representation, but lacks in providing rich semantic information of prompt $y$. When timesteps $t$ is large, the 2D diffusion model offers abundant semantic information, but its shape may not align with the current 3D representation (e.g., the orientation of people, the color of chairs, the direction of the microwave between $t$  values of 600 to 800). Continuously using smaller $t$  tends to make the generated object lean towards simple semantic information, resulting in a significant gap from the semantic cues. Conversely, continuously using larger $t$ leads to a lack of uniformity in the optimization direction of the 3D representation with each iteration, causing the shape to collapse.

\par Therefore, by hybridizing information from different 2D diffusion timesteps in each iteration, we can ensure a certain degree of shape constraint while also enriching the semantic information. For instance, in Fig.~\ref{fig:multi-timesteps}, at the $300$-th iteration phase of the man, we need to restrict the shape using the information of timesteps $t$ in $200\sim 400$, get richer semantic information
using the information of timesteps  $t$ in $400\sim 600$ and $600\sim 800$. However, at the $1000$-th iteration of the microwave, we find that the current 3D representation already possesses ample semantic information, and the information provided by larger $t$ might actually hinder the current optimization direction. Therefore, similar to DreamTime~\cite{huang2023dreamtime}, our timesteps $t$ sampling interval decreases linearly, as:
\begin{equation}
    t_i = T_{end}(iter)\cdot random(\frac{i-1}{m},\frac{i}{m}),i=1,...,m,
\end{equation}
where $iter$ represent the current iterations of the optimzation process and $m$ denotes the number of samples t.
Our HybridTime Sampling(HTS) combined with the CSD (Classifier Score Distillation)~\cite{yu2023text} method can be expressed as:
\begin{equation}
     \nabla_{\theta}\mathcal{L}_{\text{HTS}}(\theta) = \mathbb{E}_{t,\epsilon,c}\left[\sum\limits_{i=1}^{m} w(t)(\epsilon_{\phi}(x_{t_i}; y, t_i) - \epsilon_{\phi}(x_{t_i}; \emptyset, t_i))\frac{\partial g(\theta,c)}{\partial \theta}\right].
\label{equ:HTS}
\end{equation}
\par In the later stages of iteration, we can expedite the generation of plausible surface textures for the 3D representation using 3D reconstruction methods~\cite{kerbl20233d}. Through the optimization process described above, resulting in a semantically rich 3D representation, we find that when sampling very small timesteps $t$($0\sim 200$), the image $\hat{x}_{0}^t$ predicted by the Eq.~\ref{Eq:pseudoGT}
 have no difference in 3D shape compared to the image $x_0$ before noise addition, but they offer more detailed and plausible textures. Therefore, under the premise of  shape consistency, we can directly \textbf{generate} a new 3D representation through \textbf{3D reconstruction}. As shown in Fig.\ref{fig:Gen by Recon}, after obtaining a texture coarse but highly consistent 3D representation in the previous step, we render $K$ images $x_i,i=1,...,K$ from various camera poses $c_i$ around the 3D representation. By adding $t$ timesteps of noise to the images to get $x_{it}$, we estimate the images $\hat{x}_{i0}^t$ with  plausible textures using \ref{Eq:pseudoGT}, and then reconstruct them on the coarse representation through 3D reconstruction methods \cite{kerbl20233d} by minimize the following reconstruction loss:
\begin{equation}
L_{rec} = \sum_i ||g(\theta , c_i) - \hat{x}_{i0}^t||_2 .
\end{equation}
 This process, taking only \textbf{15 seconds}, generates a representation with detailed textures. 




==> supp_bbl.tex <==
\begin{thebibliography}{10}
\providecommand{\url}[1]{\texttt{#1}}
\providecommand{\urlprefix}{URL }
\providecommand{\doi}[1]{https://doi.org/#1}

\bibitem{cohen2023set}
Cohen-Bar, D., Richardson, E., Metzer, G., Giryes, R., Cohen-Or, D.: Set-the-scene: Global-local training for generating controllable nerf scenes. arXiv preprint arXiv:2303.13450  (2023)

\bibitem{hollein2023text2room}
H{\"o}llein, L., Cao, A., Owens, A., Johnson, J., Nie{\ss}ner, M.: Text2room: Extracting textured 3d meshes from 2d text-to-image models. arXiv preprint arXiv:2303.11989  (2023)

\bibitem{lin2023componerf}
Lin, Y., Bai, H., Li, S., Lu, H., Lin, X., Xiong, H., Wang, L.: Componerf: Text-guided multi-object compositional nerf with editable 3d scene layout. arXiv preprint arXiv:2303.13843  (2023)

\bibitem{ouyang2023text2immersion}
Ouyang, H., Heal, K., Lombardi, S., Sun, T.: Text2immersion: Generative immersive scene with 3d gaussians. arXiv preprint arXiv:2312.09242  (2023)

\bibitem{rombach2022high}
Rombach, R., Blattmann, A., Lorenz, D., Esser, P., Ommer, B.: High-resolution image synthesis with latent diffusion models. In: Proceedings of the IEEE/CVF conference on computer vision and pattern recognition. pp. 10684--10695 (2022)

\bibitem{vilesov2023cg3d}
Vilesov, A., Chari, P., Kadambi, A.: Cg3d: Compositional generation for text-to-3d via gaussian splatting. arXiv preprint arXiv:2311.17907  (2023)


\bibitem{zhang2024text2nerf}
Zhang, J., Li, X., Wan, Z., Wang, C., Liao, J.: Text2nerf: Text-driven 3d scene generation with neural radiance fields. IEEE Transactions on Visualization and Computer Graphics  (2024)

\bibitem{zhang2023scenewiz3d}
Zhang, Q., Wang, C., Siarohin, A., Zhuang, P., Xu, Y., Yang, C., Lin, D., Zhou, B., Tulyakov, S., Lee, H.Y.: Scenewiz3d: Towards text-guided 3d scene composition. arXiv preprint arXiv:2312.08885  (2023)

\bibitem{zhou2024gala3d}
Zhou, X., Ran, X., Xiong, Y., He, J., Lin, Z., Wang, Y., Sun, D., Yang, M.H.: Gala3d: Towards text-to-3d complex scene generation via layout-guided generative gaussian splatting. arXiv preprint arXiv:2402.07207  (2024)

\end{thebibliography}
